Relative Fukaya Categories via Gentle Algebras

Relative Fukaya categories are hard to construct. In this paper, we provide a very explicit construction in the case of punctured surfaces. The starting point is the gentle algebra $ \operatorname{Gtl} Q $ associated with a punctured surface $ Q $. Our model for the relative Fukaya category is a deformation $ \operatorname{Gtl}_q Q $ which has one formal deformation parameter per puncture. We verify that $ \operatorname{Gtl}_q Q $ is a model for the relative Fukaya category by computing a large part of the $ A_\infty $-structure on the derived category $ \operatorname{H}\operatorname{Tw}\operatorname{Gtl}_q Q $. The core method is the deformed Kadeishvili theorem from arXiv:2308.08026. The paper's technical contributions include (1) a construction for removing curvature from band objects, (2) a method for analyzing Kadeishvili trees, (3) a matching between deformed Kadeishvili trees and relative Fukaya disks. This paper is the second in a series of three, whose aim it is to deform mirror symmetry for punctured surfaces.

==> discussion/literature/barmeier.tex <==
\subsubsection{Barmeier-Wang}
\label{sec:literature-BW}
In \cite{Barmeier-Wang}, Barmeier and Wang prove the power of $ L_∞ $-morphisms in deformation theory of ordinary algebras. They depart from a quiver algebra with relations $ A = ℂQ / I $, where the ideal $ I $ is supposed to come from a reduction system. In order to classify all deformations of $ A $, they replace the Hochschild DGLA $ \HC(A) $ by a quasi-isomorphic $ L_∞ $-algebra $ L(A) $. Their line of thinking has contributed heavily to our cornerstone (O1).

%1
Barmeier and Wang study a type of quiver algebras where the ideal $ I $ comes from the act of substituting paths. Let us describe this in more detail: Let $ Q $ be a quiver and $ S $ a finite set of paths in $ Q $. Let us temporarily call a linear combination of paths $ x = λ_1 x_1 + … + λ_k x_k ∈ ℂQ $ reducible if one of the paths $ x_i $ contains an element of $ S $ as subpath. Now for every $ s ∈ S $ let $ f_s ∈ ℂQ $ be some “substitution” for $ s $. Assume that every $ f_s $ is irreducible and every $ s ∈ S $ is irreducible (except containing itself as subpath). In the words of \cite{Barmeier-Wang}, the system $ (S, \{f_s\}_{s ∈ S}) $ is then a \emph{reduction system}. The reduction system is supposed to satisfy the so-called diamond condition. Put $ I ≔ (s - f_s)_{s ∈ S} $ and define the associated quiver algebra as $ A = ℂQ / I $. In this algebra, it indeed holds that $ s $ can be substituted by $ f_s $:
\begin{equation*}
asb = a f_s b ∈ A.
\end{equation*}
To define the Hochschild DGLA, we typically use the bar resolution. Barmeier and Wang demonstrate that this resolution can be substituted by any other one, in particular the very simple bimodule resolution $ P_{\bullet} $ of Chouhy-Solotar, see \cite[Section 4.2]{Barmeier-Wang}. The cochain map between resolutions immediately gives a quasi-isomorphism of complexes
\begin{equation}
\label{eq:literature-barmeier-qi}
\Hom_{A ¤ A^{\opp}} \left(\bigoplus\limits_{i ∈ ℕ} A ¤ A^{¤_i} ¤ A, A\right) \isoto \Hom_{A ¤ A^{\opp}} (P_{\bullet}, A).
\end{equation}
The left-hand side already being a DGLA, the $ L_∞ $-structure transfer theorem induces an $ L_∞ $-structure on the right-hand side such that \eqref{eq:literature-barmeier-qi} becomes a quasi-isomorphism of $ L_∞ $-algebras.

Barmeier and Wang then compute part of the $ L_∞ $-structure on the right-hand side, just enough to classify all of its Maurer-Cartan elements. It turns out that those Maurer-Cartan elements can be exactly identified with deformations of the substitutions $ f_s $. Since Maurer-Cartan elements are preserved under the $ L_∞ $-quasi-isomorphism, this simultaneously classifies all Maurer-Cartan elements of the left-hand side $ \HC(A) $:
\begin{center}
\begin{tikzpicture}
\path (0, 0) node {deformations of $ A = ℂQ / (s - f_s)_{s ∈ S} $} (4.5, 0) node {\Large $ \longleftrightarrow $} (8, 0) node {deformations $ \tilde f_s = f_s + g_s $};
\end{tikzpicture}
\end{center}
%2
Barmeier and Wang's realization that $ L_∞ $-quasi-isomorphisms transport Maurer-Cartan elements has greatly helped us shape the curved $ A_∞ $-deformation theory of \autoref{sec:2Bainfty}. There, we make constant use of the fact that quasi-equivalences of $ A_∞ $-categories induces $ L_∞ $-quasi-isomorphisms of their Hochschild DGLAs:
\begin{equation*}
F: \cat C \isoto \cat D \quad \rightsquigarrow \quad F_*: \HC(\cat C) \isoto \HC(\cat D).
\end{equation*}
Correspondingly, their sets of Maurer-Cartan elements over any deformation base $ B $ match:
\begin{equation*}
\MCb(\HC(\cat C), B) \isoto \MCb(\HC(\cat D), B).
\end{equation*}
This is the main principle that lets us push deformations to and fro between different categories. For example, it lets us seamlessly reduce an $ A_∞ $-category to a skeleton of non-isomorphic objects without changing its deformation theory. It enable us to prove that if an object $ X ∈ \cat C_q $ is uncurvable, then all objects $ Y ∈ \cat C_q $ quasi-isomorphic to $ X $ are uncurvable as well.

%3
As aftermath of our paper, we would like to point out that Barmeier and Wang's paper is restricted to quiver algebras concentrated in degree zero with ideal given by a reduction system. Gentle algebras $ \Gtl Q $ already fall wide outside of their scope. The paper of Barmeier and Wang shows that the existence of a reduction system renders all deformations inherently straightforward. Interesting geometries will however appear as soon as we pass to algebras without reduction system or those not in degree zero. For example, the Jacobi algebra $ \Jac(Q) $ of a dimer does not possess a reduction system. It is a Calabi-Yau-3 algebra if $ Q $ is a consistent dimer. This brings $ \Jac(Q) $ into the regime of Calabi-Yau deformation theory, on which we comment in the third part of this paper series.


==> discussion/literature/keller.tex <==
\subsubsection{Keller}
\label{sec:literature-keller}
In \cite{Keller}, Keller proves that Morita equivalences of dg-categories induce $ L_∞ $-quasi-isomorphisms of the Hochschild DGLA. Thereby, Keller's work falls under cornerstone (O1).

%1
Keller regards the Hochschild DGLA not as an $ L_∞ $-algebra, but as $ B_∞ $-algebra which is slightly stronger. Let $ A $ and $ B $ be Morita equivalent dg algebras, with Morita equivalence provided by the $ A $-$ B $-bimodule $ M $. Then Keller's core argument for invariance is as follows: Embed $ A $ and $ B $ into the triangular dg algebra
\begin{equation*}
D ≔ \begin{pmatrix} A & M \\ 0 & B \end{pmatrix}.
\end{equation*}
Both embeddings $ A, B ⊂ D $ turn out to be Morita equivalences. Keller exploits the natural restriction maps $ \HC(D) → \HC(A) $ and $ \HC(D) → \HC(B) $, which automatically respect the $ B_∞ $-structure. Departing from the knowledge that Hochschild cohomology of dg algebras is invariant under Morita equivalences as graded vector space, Keller concludes that both $ \HC(D) → \HC(A) $ and $ \HC(D) → \HC(B) $ are $ B_∞ $-quasi-isomorphisms. Correspondingly, $ \HC(A) $ and $ \HC(B) $ are $ B_∞ $-quasi-isomorphic.

%2
Unfortunately, Keller's result is currently restricted to the case dg algebras. To the present paper, this means that we simply assume as axioms that the theory extends to all $ A_∞ $-categories.

%3
The heavy use of $ A_∞ $-deformations in our paper shows how imperative it is to extend Keller's paper to the $ A_∞ $-context. According to private communication with Keller, these results can likely be obtained by the same triangular construction together with appropriate $ A_∞ $-bimodule theory.

==> subdisk/test_minmodel.tex <==
\begin{theorem}
\label{th:subdisk-minmodel-th}
Let $ Q $ be a geometrically consistent dimer. Regard its category $ \DefZigzagCat ⊂ \Tw\Gtl_q Q $ of deformed zigzag paths according to \autoref{conv:alpha0-direction}. Then the minimal model $ \H\DefZigzagCat $ is described as follows:
\begin{itemize}
\item The objects are the zigzag paths of $ Q $.
\item Let $ L_1 $ and $ L_2 $ be zigzag paths. Then a basis for the hom space $ \Hom_{\H\DefZigzagCat} $ is given by the cohomology basis elements $ h: L_1 → L_2 $.
\item The $ A_∞ $-products satisfy the identities
\begin{align*}
μ^1_{\H\DefZigzagCat} &= 0, & μ^2_{\H\DefZigzagCat} \left(h, \sum_a \id_a \right) &= h \\
μ^{≥3}_{\H\DefZigzagCat} \left(…, \sum_a \id_a, …\right) &= 0, & μ^2_{\H\DefZigzagCat} \left(\sum_a \id_a, h\right) &= (-1)^{|h|} h.
\end{align*}
Let $ N ≥ 2 $ and let $ h_1, …, h_N $ be a sequence of non-identity basis morphisms with $ h_i: L_i → L_{i+1} $. Then their product is given by
\begin{equation*}
μ^N (h_N, …, h_1) = \sum_{\substack{D ∈ \CRd \disjoint \IDd \disjoint \DSd \disjoint \DWd \\ D \text{ has inputs } h_1, …, h_N}} (-1)^{\Abouzaid(D)} \punctures(D) \disktarget(D).
\end{equation*}
\end{theorem}

